Optimizing Ordered Graph Algorithms with GraphIt

Many graph problems can be solved using ordered parallel graph algorithms that achieve significant speedup over their unordered counterparts by reducing redundant work. This paper introduces a new priority-based extension to GraphIt, a domain-specific language for writing graph applications, to simplify writing high-performance parallel ordered graph algorithms. The extension enables vertices to be processed in a dynamic order while hiding low-level implementation details from the user. We extend the compiler with new program analyses, transformations, and code generation to produce fast implementations of ordered parallel graph algorithms. We also introduce bucket fusion, a new performance optimization that fuses together different rounds of ordered algorithms to reduce synchronization overhead, resulting in $1.2\times$--3$\times$ speedup over the fastest existing ordered algorithm implementations on road networks with large diameters. With the extension, GraphIt achieves up to 3$\times$ speedup on six ordered graph algorithms over state-of-the-art frameworks and hand-optimized implementations (Julienne, Galois, and GAPBS) that support ordered algorithms.

==> compiler_vldb.tex <==
\section{Compiler Implementations}
\label{sec:compiler}

\begin{figure}[!t]
\includegraphics[width=\columnwidth]{figures/OG_compiler_organization.pdf}
\caption{Changes for ordered graph processing support in \graphit.}
\label{fig:compilerorg}
\end{figure}

In this section, we describe extensions to the GraphIt compiler. An illustration is shown in Figure~\ref{fig:compilerorg}. 
We extended the frontend both for the algorithm and the scheduling language, added different program transformations and analyses to the midend, and expanded the runtime library to enable the backend to generate efficient code for ordered graph algorithms.

% Needs to be rewrote significantly. 

\punt{

% this information is repeated in the subsequent sections, let's leave them to later
The framework is implemented as an extension to the Graphit compiler~\cite{graphit:2018}. Since the programming model extends the language, new features and analyses need to be added to the frontend, midend, code generation and the runtime system. The new framework needs to capture abstractly the ordered computations from the algorithm language, transform it according to the different optimization selected in the scheduling language and then lower it to generate efficient code that makes use of multiple runtime libraries. While transforming the code for efficiency, the compiler also has to check for applicability of different schedules and argue for the correctness of the transformations. }

\punt{

\subsection {Program Analysis}

We add new program analysis passes to the GraphIt compiler midend to extract high-level semantic information from the user-defined functions, and generate code after transforming them according to the strategies chosen in the schedule. 
The frontend parses and creates midend intermediate representation (IR) nodes for the new priority queue related data types and function calls. 
These IR nodes are lowered into specialized nodes based on user specified schedules.
%Then the user-specified schedule is attached to statements and the corresponding IR nodes are transformed and specialized into optimization specific nodes. 
%\julian{the IR node representation should be defined first}
Some optimizations also require global transformations outside the scope of the statement that the schedule was applied to.
%\punt{\julian{remove second part of sentence? this requires knowledge of the node representation and what the CFG is}}

Schedules are applied to the \texttt{applyUpdatePriority} operator as shown in  Lines~\ref{line:delta_stepping_apply_update_priority_start}--\ref{line:delta_stepping_apply_update_priority_end} of Figure~\ref{fig:code:delta_stepping_GraphIt}. 
The schedules control the priority update strategy for the vertices in the priority queue, while also specifying other related parameters like $\Delta$ size or bucket fusion threshold. 

The program analysis passes in the PriorityFeaturesLower stage map relevant schedules to the applyUpdatePriority nodes. This information is then propagated to the vertex sets, the priority queue, and other related data structures. 
Different optimization decisions require different representations of these intermediate data structures when generating code. 
For instance, Figure~\ref{fig:code:julienne_graph_load} shows how the priority queue is created when the lazy priority update method is used. 
This is because the implementation uses the Julienne~\cite{Dhulipala:2017} framework in the runtime library for the lazy priority queue. On the other hand, the eager priority update method generates code as shown in Figure~\ref{fig:code:gapbs_graph_load}. \punt{ \julian{could have more explanation on what the parameters of the code are doing}}


\begin{figure}


% \lstset{numbers=left, numberstyle=\tiny, stepnumber=5,%
% numberfirstline=false, numbersep=5pt}

%\lstset{language=C++,backgroundcolor=\color{lightbackground},%belowskip=.5em, aboveskip=.5em, stepnumber=1, numberfirstline=true}

\begin{lstlisting}[language=C++,escapechar=|]
pq = new PriorityQueue <int> ( edges.n,
    Distance, //Priority array 
    increasing, //bucket_order
    strictly_decreasing, //priority_order
    128); // Number of buckets
\end{lstlisting}



\caption{\graphit generated code for constructing lazy update priority queue.}
\label{fig:code:julienne_graph_load}
\end{figure}

\begin{figure}
\if 0
\begin{lstlisting} [language=c++,escapechar=|]
edges = builtinLoadEdgesFromFile("...");
\end{lstlisting}
\fi

\begin{lstlisting} [language=c++,escapechar=|]
pq = new EagerPriorityQueue <int > ( 
    Distance, // Priority array
    2); // Delta size
\end{lstlisting}

\caption{\graphit generated code for for construction eager update priority queue}
\label{fig:code:gapbs_graph_load}
\end{figure}

In order to support optimizations like switching to thread-local eager queue implementations, we need to change the control flow of the program. We add analysis passes to identify such patterns and uncover more opportunities for optimizations. This analysis enables the UDF transformation passes to gather the required parameters from the algorithm.
For example, Lines~\ref{line:ordered_processing_operator_start}--\ref{line:ordered_processing_operator_end} in Figure~\ref{fig:code:delta_stepping_GraphIt} have a pattern where the vertices in the buckets are processed in priority order until all the vertices are processed. 
These IR nodes are collapsed into a single OrderedProcessingOperatorWithMerge operator as shown in Figure~\ref{fig:code:delta_stepping_ordered_processing_call}. Notice how we extract the loop conditions and other parameters like the start vertex from the while loop and pass them as parameters to the newly created operator. This transformation is required to enable more parallelization strategies and maintain thread-local data structures across iterations in the case of the bucket fusion optimization. 


\begin{figure}[!t]
\begin{lstlisting} [language=c++,escapechar=|]
...
OrderedProcessingOperatorWithMerge(pq, 
    edges, [&]()->bool{return ((pq->finished() ) == 
        ((bool) 0));}, 
    updateEdge(), 1000, start_vertex);
...
\end{lstlisting}
\caption{While loop from \deltastepping{} collapsed into a single OrderedProcessingOperatorWithMerge node.}
\label{fig:code:delta_stepping_ordered_processing_call}
\end{figure}
}


\subsection {User-Defined Function Transformations}

The compiler transforms the user-defined functions in the algorithm language to support different performance optimizations such as eager and lazy bucket updates, and parallelization. 
\punt{
% a piece of detail provided too early
The user defined functions supplied to the applyUpdatePriority operator call the updatePriority class of functions to update the priority of a single node in the priority queue. But depending on the schedule used, the updates to the priority might not happen immediately. }

% eager UDF transformation, tall about this one first because KCore optimization is not fully described in the programming section, will be a bit confusing. 
In order to apply the eager bucket update optimization, additional arguments need to be supplied
to the user-defined functions. The eager bucket update approach uses thread-local buckets 
that are hidden from the user and cannot be stored in the global priority queue. 
As a result, we append the local buckets to the argument list for the user-defined update functions 
and the priority update functions. 
This way, we are able to generate code that can eagerly update thread-local buckets 
from high-level priority update abstractions. 

% lazy UDF transformation
For \kcore{}, the best schedule uses the lazy bucket update approach. Since the priorities for each vertex always reduce by 1 at each update, we can optimize it further by gathering only the number of updates to each vertex and then updating the priority of the vertex in a single step. 
\punt{This optimization is specified in the schedule as the constant\_sum\_reduce\_before\_update.}
We write an analysis pass as part of the PriorityFeaturesLower stage that performs pattern matching on the body of the user-defined function to determine whether the change to the priority of the vertex is a fixed value. 
It then extracts this delta and other related parameters like the expressions for the minimum priority. The actual \textsf{apply} operator then gets only the counts of updates to each vertex and calculates the change in priority for each vertex. \punt{finally updates the nodes by multiplying the extracted delta to the update count for each node. \julian{why multiplying?}} The original user-defined function is shown in Figure~\ref{fig:code:kcore_udf_original} and the transformed function and the update to the buckets generated is shown in Figure~\ref{fig:code:kcore_udf_updated}. We have to ensure that all the expressions used in the operator and the expressions that they depend on are copied into the transformed function. 
This transformation allows the user to write the \textsf{apply} function with the same interface irrespective of the schedule while using the most efficient implementation to generate code. 

\begin{figure}[!t]
\begin{lstlisting} [language=graphit]
func apply_f(src: Vertex, dst: Vertex)
    var k: int = pq.get_current_priority();
    pq.updatePrioritySum(dst, -1, k);
end
\end{lstlisting}
\caption{The original user-defined function for updating priorities in \kcore{} written in \graphit.}
\label{fig:code:kcore_udf_original}
\end{figure}

\begin{figure}[!t]
    \begin{lstlisting} [language=c++,escapechar=|]
apply_f_transformed = [&] (const tuple<unsinged int, 
unsinged int> &p) {
    int k = pq->get_current_priority() ;
    NodeID node = std::get<0>(p);
    unsigned int count = std::get<1>(p);
    if ( D[node] > k) {
      unsigned int __new_pri = std::max(D[node] +  (-1)   * count, (unsigned int)(k));
      D[node] = __new_pri;
      return wrap(node, pq->get_bucket(__new_pri));}}
      
    \end{lstlisting}
    \caption{The transformed user-defined function for updating priorities in \kcore{}.}
    \label{fig:code:kcore_udf_updated}
\end{figure}




\subsection {Code Generation}
Code generation materializes the optimized and transformed IR nodes
into C++ programs.
\punt{All the optimizations and the transformation described in the previous sections are actually materialized in the code generation phase.}
We generate appropriate code to iterate over the vertices and edges and use different data structures from the runtime library as prescribed by the schedule. 
We also insert specialized statements for a specific schedule or optimization strategy (for example, the bulk\_update\_buckets call in case of lazy bucket updates as shown on Line~\ref{line:bulk_bucket_update} of Figure~\ref{alg:lazy_delta_stepping}). \punt{\julian{not sure where update\_buckets is defined} }
We describe these code generation changes in this section. 
The program analysis passes determine the correct specialization for each of the IR nodes depending on the choice of the optimizations specified in the schedules. This specialization is applied to the \textsf{apply} operators, the vertex set types, and the priority queue types.
%too vague
\punt{he passes also create new data structures for certain schedules like the EdgeMap data structure required by the lazy priority update optimization. }

\punt{Code generation leverages the analyses from the midend to generate the right data structures to use the appropriate runtime library.}

Code generation also bridges the gap between the optimization decisions and the rich functionality from the runtime library.
The runtime library has multiple implementations of the same data structure suitable for different schedules. 
Depending on what optimizations are enabled and the context of the expression, we use the right representation or insert calls to appropriate runtime libraries. 
% \punt{If a certain representation is not required in the computation, we do not materialize the representation to avoid overallocation and superflous computations. All these decisions are made in the code generation phases. }
% \punt{The midend passes depending on the schedules specified attach appropriate context information to each IR node. }
For example, the eager bucket update method requires that the eager bucketing data structures and the priority\_queue constructor is lowered into a call to EagerPriorityQueue() from the runtime library when this schedule is specified.
% \punt{as apposed to a call to julinne::priority\_queue() when the lazy update schedule is specified on the applyUpdatePriority operator.} 
This decision process in the code generation phase allows the programmer to use a common representation in the algorithm language across different scheduling options. 
Similar specializations are done for the vertex set data structures depending on the schedule. 

% Won't talk about extern functions since we don't have space
%\punt{Real world applications that implement complicated algorithms which require functions that are not currently supported in the GraphIt runtime and are difficult to implement in the language itself. We extend the compiler to give the programmer the flexibility to link GraphIt generated code with external C++ code. }
%
%Some graph applications require functions that are not related to graph 
%operations. To support these applications, we extend the compiler to link  generated code with external C++ code. 
%This feature is useful for writing complicated UDFs and using custom graph loaders as in the case of \astar{}. The algorithm language is extended to add the \texttt{extern} keyword before function declarations. The function declarations can have \graphit types for arguments and the return type. For the functions declared as \texttt{extern}, the compiler does not generate a function body but only inserts a forward declaration of the function with the \graphit types substituted with equivalent C++ types. The user can write the body of the functions in a separate source file. The \texttt{extern} functions have access to all the global variables declared in the \graphit code apart from the arguments. 
%The \graphit compiler cannot analyze and transform the body of the \texttt{extern} functions, so the programmer has to take care of synchronization and performance for the \texttt{extern} functions. 
%
%\punt{ Mainly -
%\begin{itemize}
%    \item The user has to ensure that the extern function is not called from any performance critical sections of the algorithm, since they will lose on optimization opportunities. 
%    \item Since the compiler cannot do dependence analysis on the body of the function, the user has to ensure that appropriate synchronization primitivies are added to the function if it is invoked from parallelized regions of code. 
%\end{itemize}
%We use the extern functions in this paper in the \astar{} application to load the coordinates of the vertices in the graph from a custom data format and to calculate the pairwise non-euclidean distance for intializing the priorities. 
%\if 0
%There are many global program transformations that needs to be happen in order to switch between different schedules. 
%The compiler reads the schedules assigned to the applyUpatePriority, and then generates the right type for priority queue (thread-local) or global. 
%If lazy update, the priority updates are buffered and vertices whose priority are updated are materialized into a frontier. 
%Additional operators to insert into the priority queue needs to be generated as well. 
%Need to replace the while loop with an ordered processing operator. 
%\fi
%}

\subsection{Runtime Libraries}
\label{sec:runtime_lib}

We designed a set of runtime libraries to implement the eager bucket update, eager bucket update with bucket fusion, and lazy bucket update optimizations. 

For eager bucket updates, we developed efficient libraries for the priority queue, thread-local bucket updates 
and bucket retrieval, and ordered processing operators. 
The global priority queue keeps track
of the vector that holds the priority values, delta, and the current priority. It can perform appropriate priority and bucket updates and keep track of status of the computations.  

\punt{The priority queue also provides the API to check if all the buckets have been processed (\texttt{priority\_queue.finished()} ), or if a particular
node has finished processing by checking the priority of the node with the current priority (\texttt{priority\_queue.finishedNode(v)}). }

We use an ordered processing operator for eager bucket updates. This operator uses OpenMP parallel regions to set up the thread-local buckets. 
The operator supplies a while loop inside to perform the iterative processing across all of the buckets. 
In each iteration of the while loop, the operator distributes work among the different threads, synchronizes across threads to enforce priority ordering, and merges local buckets into a global bucket on every round. 
The bucket fusion optimization adds another while loop nested inside
the outer while loop in the ordered processing operator. 


\punt{
At the beginning of each round of the while loop, 
the operator uses OpenMP parallel for loop on a global bucket 
that contains vertices of the current priority with 
work-stealing to redistribute the work across the different threads. 
Once the global bucket is formed, the transformed user defined functions are used to update the 
priorities of the nodes. Atomic synchronizations are used 
to ensure atomicity on the priority updates. 
At the end of the round, it uses one global synchronization to find
the next priority, and each thread subsequently copies 
their local bucket of the next priority into the global bucket. 

The bucket fusion optimization adds another while loop nested inside
the outer while loop in the ordered processing operator. In this nested 
while loop, it first makes a copy of the next lowest priority bucket, 
and then processes it if the next bucket is of the same priority 
as the current bucket and the size of the next bucket is less
than a threshold. }

For lazy bucket updates, we use a prefix sum to implement the bucket update buffer without relying on atomics, and use the bucketing structure from Julienne~\cite{Dhulipala:2017}. 
We allocate an array to hold the bucket update for each 
edge that we process. 
Since not all of the edges will result in a bucket update, we 
use a prefix sum across the allocated array to collect all the updates together in a new buffer. 
For \kcore{}, the buffer reduction is specialized with a histogram approach.
%\julian{is this a histogram instead of a prefix sum? on KCore uses a histogram} 
This lets us avoid the overhead of atomic synchronization when appending bucket updates to the buffer. 
The priority-based buckets only materialize a fixed number of buckets, and store the rest of the 
vertices in an overflow bucket. 
%\julian{should stick to using "bucket" instead of introducing a new term "bin". i think bin was used earlier without being defined. check table 2 also. DONE}
More bins are created from the overflow bin when the previously
materialized bins are processed. 
We provide a scheduling API to tune 
the number of bins that are materialized. 
%not for now
\punt{
\ajay {should we insert a figure here to show the buckets?}}


\punt{

The ordered graphit runtime library is a fusion of the GAPBS~\cite{DBLP:journals/corr/BeamerAP15} and the Julienne~\cite{Dhulipala:2017} runtime libraries.

The Julienne runtime library is wrapped up inside the julienne namespace to avoid name conflicts with the Ligra~\cite{shun13ppopp-ligra} runtime library and to maintain compatibilty with the optimizations from the original \graphit work. The code generator is aware of this and uses the julienne namespace only in the context of the ordered operators.

We wrote wrappers around these libraries to expose a similar interface to the applications. 

The builtins from the original \graphit library like
getVertices() or getDegrees() have been overloaded to accept the new graph types so that the code generator can use the same builtins with the new representations. This simplifies code generation in most cases.

We constructed our ordered processing operator from GAPBS operator, we use Julienne for our buffered update. 

We use OpenTuner to tune the scheduling and parameters for delta, number of bins. 

\subsection {Autotuner}
}
